Payment Networks as Creation Games

Payment networks were introduced to address the limitation on the transaction throughput of popular blockchains. To open a payment channel one has to publish a transaction on-chain and pay the appropriate transaction fee. A transaction can be routed in the network, as long as there is a path of channels with the necessary capital. The intermediate nodes on this path can ask for a fee to forward the transaction. Hence, opening channels, although costly, can benefit a party, both by reducing the cost of the party for sending a transaction and by collecting the fees from forwarding transactions of other parties. This trade-off spawns a network creation game between the channel parties. In this work, we introduce the first game theoretic model for analyzing the network creation game on blockchain payment channels. Further, we examine various network structures (path, star, complete bipartite graph and clique) and determine for each one of them the constraints (fee value) under which they constitute a Nash equilibrium, given a fixed fee policy. Last, we show that the star is a Nash equilibrium when each channel party can freely decide the channel fee. On the other hand, we prove the complete bipartite graph can never be a Nash equilibrium, given a free fee policy.

==> single.tex <==
\section{Single Channel}
In this section, we study the online problem of finding a profitable strategy of accepting and rejecting incoming transactions (at most $n$) given capital constraints as defined in \cite{Avarikioti2018algorithmic}, i.e. we consider the online version of Problem \ref{Single Channel}. First, we discuss the existence of competitive algorithms against different adversarial models. Next, we show lower bounds on the advice bits needed for competitive deterministic algorithms with advice. 
%The advice complexity of such algorithms often shows the difficulty of online problems and is used to bound the expected competitive ratio of randomised algorithms from below. This technique was used for the analysis of various problems \cite{BOCKENHAUER201461, CSIRIK2002308, osti_471379, Komm:2016:IOC:3036138}. 
The competitiveness is analysed from two perspectives: maximising the number of accepted transactions and minimising the number of rejected transactions, both of which imply the maximisation of the PSP's profit. Therefore, we examine the advice complexity for two different but similar definitions of the competitive ratio. Then, we use the relationship between advice and randomisation to discuss the competitiveness of randomised online algorithms. Last, we consider resource augmentation, i.e. we assume an online algorithm has more resources (more capital on both sides) than an optimal offline algorithm.

%---------------RANDOMIZED-------------------------------
\subsection{Lower bounds for randomized algorithms}
As proven in \cite{Avarikioti2018algorithmic}, competitive deterministic algorithms against adaptive adversaries do not exist. We show that there are no randomised algorithms against adaptive adversaries.

\begin{theorem}
    There is no competitive randomised algorithm against adaptive adversaries.
\end{theorem}
\begin{proof}
	Assume that there is a competitive randomised algorithm against any adaptive online adversary.
	Theorem 2.1 and Theorem 2.2 in \cite{Ben-David90onthe} state that the existence of a randomised $c$-competitive algorithm against any adaptive online adversary and the existence of a randomised $d$-competitive algorithm against any oblivious adversary imply the existence of a $cd$-competitive randomised algorithm against any adaptive offline adversary. Additionally, this implies that there is a $cd$-competitive deterministic algorithm. Since a $c$-competitive algorithm against any adaptive online adversary is $c$-competitive against any oblivious adversary, the existence of a $c$-competitive randomised algorithm against any adaptive online adversary implies the existence of a $c^2$-competitive deterministic algorithm.
	From Theorem 19 in \cite{Avarikioti2018algorithmic} we know that there are no deterministic online algorithms against adaptive online adversaries which contradicts our assumption and proves that there is no competitive randomised algorithm.
\end{proof}

From here on, we discuss algorithms against oblivious adversaries since there are no algorithms against stronger adversaries. We show that a greedy algorithm performs poorly. Then, we prove that there is no competitive deterministic algorithm against oblivious adversaries to illustrate the importance of the analysis of randomised algorithms against oblivious adversaries.

\begin{theorem}
    Greedy algorithms are not competitive.
\end{theorem}
\begin{proof}
    A greedy strategy is accepting all incoming transactions that are executable. We present the following sequence of transactions with given initial capital distribution $\langle n-1;0\rangle$:
    $$(l,r,n-1),(l,r,1),(l,r,1), \dots, (l,r,1)$$
	Accepting the first transaction generates a new capital distribution $\langle 0;n-1 \rangle $. Thus, the greedy algorithm cannot accept subsequent transactions. In opposition, the optimal offline algorithm rejects the first transaction and accepts all others. This gives a competitive ratio of $c = \frac{n-1}{1} = n-1 \in \theta(n)$.
\end{proof}

\begin{theorem}
	There is no competitive deterministic algorithm against any oblivious adversary.
\end{theorem}
\begin{proof}
	Suppose the initial capital distribution is $\langle n;1 \rangle $. We present the following sequences of transactions:
	\begin{enumerate}
		\item $(l,r,n-1),(r,l,1),(l,r,n+1),(r,l,n+1),(l,r,n+1),(r,l,n+1),\dots$
		\item $(l,r,n-1),(r,l,n),(l,r,n+1),(r,l,n+1),(l,r,n+1),(r,l,n+1),\dots$
	\end{enumerate}
	An algorithm must reject the first transaction such that it is competitive on the first sequence of transactions. Otherwise, the whole capital cannot be on one side such that the movement of it back and forth cannot be accepted. Thus, if a deterministic algorithm exists, it must reject the first transaction. For the second sequence of transactions, the whole capital cannot be on one side if the first transaction is rejected. Then, the movement of the total capital back and forth is not possible. Consequently, there is no competitive deterministic algorithm.
\end{proof}

%---------------ADVICE-------------------------------
\subsection{Algorithms with advice}

\subsubsection{Maximising the Number of Accepted Transactions}
Since maximising the number of accepted transactions enlarges the profit, we consider algorithms maximising the number of accepted transactions. We define the competitive ratio of an algorithm $ALG$ to be a value $c$ such that the ratio between the number of accepted transactions by the optimal offline algorithm $OPT$ and $ALG$ for all input sequences $I_x$ is less than or equal to $c$: $$\forall x. c \geq \frac{OPT(I_x)}{ALG(I_x)}$$
In this section, we study deterministic algorithms with advice, i.e. we show how many advice bits are needed for an algorithm to be optimal. 
%Then, we derive results for randomised algorithms.

\begin{theorem}
    An optimal algorithm reading $n-2$ advice bits exists.
\end{theorem}
\begin{proof}
    The advice gives the strategy for the first $n-2$ transactions. For the last two transactions, the algorithm proceeds greedily. If the optimal offline algorithm accepts none of the last two transactions, none of them can be accepted. If one or two transactions can be accepted, our algorithm will accept and reject them accordingly such that it is optimal.
\end{proof}
    
\begin{theorem}
    There is no optimal algorithm reading less than $n-2$ advice bits.
\end{theorem}
\begin{proof}
    Assume an algorithm $ALG$ reading at most $n-2$ advice bits exists. Then, $ALG$ reads no advice bits for $n=3$. We construct following sequences of transactions with initial capital distribution $\langle 2;1 \rangle $:
    \begin{enumerate}
        \item ($l,r,2$),($l,r,1$),($l,r,1$)
        \item ($l,r,2$),($r,l,3$),($r,l,3$)
    \end{enumerate}
    For the second sequence of transactions, the optimal offline algorithm accepts the first transaction, whereas, for the first sequence, the first transaction is rejected. Since $ALG$ is deterministic, the decision made on the first transaction will always be the same. Consequently, $ALG$ cannot be optimal.
\end{proof}    

Since the number of advice bits needed for an optimal solution is high, we consider approximation algorithms, i.e. the competitive ratio can be greater than one. Therefore, we show lower bounds on advice bits for different competitive ratios. 
%A common technique is to construct a set of inputs with a common prefix and to show that for each element in the set a unique strategy on the prefix is required such that the solution is competitive. Usually, this is done using the pigeonhole principle. This technique is used to show lower bounds on advice bits in the online knapsack problem \cite{BOCKENHAUER201461} and is described in \cite{Boyar2016OnlineAW}. Our goal is to construct a set of sequences of transactions with a shared prefix to show a lower bound on the advice bits needed.

\begin{theorem}
    An algorithm reading strictly less than $f(n)$ advice bits has a competitive ratio of $\Omega(\frac{n}{f(n)})$.
\end{theorem}
\begin{proof}
    Let the initial capital distribution be $\langle 2^{f(n)};1 \rangle$ and $f(n)$ be a function such that $f(n) \in o(n)$. $loop$ denotes transactions that move the total capital from left to right until there are $n$ transactions. We define a sequence of transactions as $$I_x = (l,r,1), \dots, (l,r,2^{f(n)-1}), (r,l,x+1), loop$$ such that the set of instances is defined as $$\mathcal{I} = \{I_x \mid x \in \{0, \dots, 2^{f(n)}-1\}\}$$
    Similar to the proofs before, an algorithm must accept $loop$, otherwise the competitive ratio is $c \geq \frac{n-f(n)}{f(n)+1}$. Assume that there is an algorithm $A$ reading at most $k < f(n)$ advice bits. For instance $I_x$, $A$ must transfer $x$ capital with the transactions of the prefix to the right side such that it can accept $loop$. The number of strategies the advice can describe is smaller than the number of instances in the constructed input set. Thus, we know that for two different inputs the same strategy is used. We conclude, $A$ cannot accept $loop$ for one element in $\mathcal{I}$ and has competitive ratio $c \geq \frac{n-f(n)}{f(n)+1}$.
\end{proof}

\subsubsection{Minimising the Number of Rejected Transactions}
In the previous subsection, we defined the competitiveness as the ratio between the number of accepted transactions of the optimal offline algorithm and an online algorithm which was an online maximisation problem. In this section, we examine the problem from another point of view. Namely, we define the competitive ratio such that it is a minimisation problem. Consequently, we say the competitive ratio for minimising the number of rejected transactions for an online algorithm $ALG$ is a value $c$ such that: $$\forall x. c \geq \frac{ALG(I_x)}{OPT(I_x)}$$
$ALG(I_x)$ and $OPT(I_x)$ describe how many transactions are rejected by the respective algorithm for the input sequence $I_x$. The methodology and results are closely related to what we have seen in the previous section. First, we consider deterministic algorithms with advice and prove a general lower bound on the advice bits needed for a general competitive ratio. Then, we proceed with giving lower bounds on the competitiveness for randomised algorithms.

\begin{theorem}\label{minRejectedAdvice}
    An algorithm reading strictly less than $f(n)$ advice bits has a competitive ratio of $\Omega(\frac{n}{f(n)})$.
\end{theorem}
\begin{proof}
    Let $\langle 2^{f(n)};1\rangle$ be the initial capital distribution.
    We define $$\mathcal{I} = \{I_x \mid x \in \{0,\dots,2^{f(n)}-1\}\}$$ where $$I_x = (l,r,1), (l,r,2),\dots(l,r,2^{f(n)-1}), (r,l,x+1), loop$$ for $f(n) \in o(n)$ and $loop$ being a sequence of transactions moving all the capital from left to right back and forth. An algorithm that does not accept $loop$ has a competitive ratio of at least $c \geq \frac{n-f(n)-1}{f(n)}$. Assume there is an algorithm reading $k < f(n)$ advice bits with a better competitive ratio. Since there are $2^{f(n)}$ different instances in $\mathcal{I}$ and fewer strategies are expressible by the advice, one strategy is used for two elements of the input set. In the previous section, we showed that transferring $i$ is the only strategy accepting $loop$ for an instance $I_i$. Then, for $I_j$ where $j \neq i$ the strategy that transfers $i$ with the transactions of the prefix cannot accept $loop$. As a result, the competitive ratio is at least $c \geq \frac{n-f(n)-1}{f(n)}$ which contradicts the assumption that there is an algorithm with a better competitive ratio reading $k < f(n)$ advice bits.
\end{proof}



%---------------ADVICE TO RANDOM----------------------
\subsection{From advice to randomization}

\subsubsection{Maximising the Number of Accepted Transactions}

In this section, we show lower bounds on the competitiveness of randomised algorithms using our results on algorithms with advice, since algorithms with advice and randomised algorithms are closely related. According to  \cite{Borodin:1998:OCC:290169}, Yao's Principle \cite{yao1977probabilistic} bounds the expected competitive ratio of randomised algorithms from below with
$$R \geq max\left(min_i \frac{\E_{y(j)}[OPT(\sigma_j)]}{\E_{y(j)} [ALG_{i}(\sigma_j)]}, min_i \frac{1}{\E_{y(j)}[\frac{ALG_i(\sigma_j)}{OPT(\sigma_j)}]}\right)$$
where both arguments in the maximum function are proven lower bounds. $\E[X]$ is the expectation of a random variable $X$. $OPT$ is the optimal offline algorithm and $ALG_i$ is the optimal strategy for the input sequence $\sigma_i$. $y(j)$ is the distribution of $j$ and $\sigma_j$ is an input sequence for all $j$. We use $c$ for the expected competitive ratio and $I_x$, as before, for the input sequences. We change the other variables accordingly.

\begin{theorem}
    A randomised online algorithm is $\Omega(\frac{n}{f(n) + \frac{n}{2^{f(n)}}})$-competitive for the single channel case.
\end{theorem}
\begin{proof}
    Let $\langle 2^{f(n)};1 \rangle $ be the initial capital distribution and $$\mathcal{I} = \{I_x \mid x \in\ \{0,\dots,2^{f(n)}-1\}\}$$ the set of sequences of transactions for $f(n) \in o(n)$ where $$I_x = p, (r,l,x+1), loop$$ and $p = (l,r,1), (l,r,2), \dots, (l,r,2^{f(n)-1})$. $loop$ is the movement of the capital back and forth. Then, we define the set of strategies as $\mathcal{A} = \{A_x \mid x \in \{0, \dots, 2^{f(n)}-1\}\}$. 
    A non-optimal strategy accepts at most $f(n)$ transactions, whereas the optimal strategy accepts at most $n$ and at least $n-f(n)$ transactions. We will refer to this in the following calculation as $(*)$. 
    \begin{align*}
        c & \geq min_i \frac{1}{\E_{y(j)}[\frac{A_i(I_j)}{OPT(I_j)}]} & \mbox{Yao's principle} & \\
        & = \frac{1}{max_i \E_{y(j)}[\frac{A_i(I_j)}{OPT(I_j)}]}&\\
        & \geq \frac{1}{max_i \E_{y(j)}[\frac{A_i(I_j)}{n-f(n)}]} & \mbox{$OPT(I_j) \geq n-f(n)$}&\\
        & = \frac{n-f(n)}{max_i \E_{y(j)}[A_i(I_j)]}&\\
        & \geq \frac{n-f(n)}{\sum\limits_{k=0, k \neq i}^{2^{f(n)}-1} (\frac{1}{2^{f(n)}}(f(n)+1)) + \frac{n}{2^{f(n)}}}&\mbox{$y(j)$ uniform and $(*)$}&\\
        & = \frac{n-f(n)}{(2^{f(n)}-1)(\frac{f(n)+1}{2^{f(n)}}) + \frac{n}{2^{f(n)}}}&\\
        & = \frac{n-f(n)}{f(n) + 1 - \frac{f(n)+1}{2^{f(n)}} + \frac{n}{2^{f(n)}}}&\\
        & \geq \frac{n-f(n)}{2(f(n) + \frac{n}{2^{f(n)}})}&\\
    \end{align*}
    Thus, we have shown that $c \in \Omega(\frac{n}{f(n) + \frac{n}{2^{f(n)}}})$.
\end{proof}

We showed a general lower bound on the expected competitive ratio of a randomised algorithm. Finding a function that minimises the asymptotic growth of $f(n) + \frac{n}{2^{f(n)}}$ gives us a high lower bound. We examined the case where $f(n) = \log(n)$ which gives already a high lower bound. We conclude that there are no randomised algorithms with a good competitive ratio.

\subsubsection{Minimising the Number of Rejected Transactions}
Similarly to the randomised maximisation of the number of accepted transactions, we can bound the expected competitive ratio of randomised algorithms for minimisation problems using the relationship between advice and randomisation. As stated in section 8 in \cite{Borodin:1998:OCC:290169}, Yao's Principle \cite{yao1977probabilistic} bounds the expected competitive ratio for minimisation problems from below with
$$\bar{R} \geq max\left(min_i \frac{\E_{y(j)} [ALG_{i}(\sigma_j)]}{\E_{y(j)}[OPT(\sigma_j)]}, min_i \E_{y(j)}[\frac{ALG_i(\sigma_j)}{OPT(\sigma_j)}]\right)$$
where both arguments in the maximum function are proven lower bounds. The notation is the same as in section \ref{maximRandom}.
\begin{theorem}\label{minRejectedRandom}
    A randomised algorithm minimising the number of rejected transactions is $\Omega(\frac{n}{f(n)})$-competitive.
\end{theorem}
\begin{proof}
    We construct the same set of instances as in the proof of Theorem \ref{minRejectedAdvice} with the same initial capital distribution. Accordingly, we define the set of strategies to be $\mathcal{A} = \{A_x \mid x \in \{0,\dots,2^{f(n)}-1\}\}$ where $A_x$ is the optimal strategy for $I_x$. As discussed in previous proofs, choosing a non-optimal strategy for an input results in the rejection of at least all of the $n-f(n)-1$ transactions in $loop$. We know that the optimal offline algorithm rejects at most $f(n)$ and at least no transactions.
    
    \begin{align*}
        c & \geq \min_i \frac{\E_{y(j)}[A_i(I_j)]}{\E_{y(j)}[OPT(I_j)]}&\mbox{Yao's Principle}&\\
        & \geq \min_i \frac{\E_{y(j)}[A_i(I_j)]}{f(n)}&\\
        & = \min_i \frac{\sum_{j=0,j \neq i}^{2^{f(n)}-1} ( A_i(I_j)) + OPT(I_j)}{2^{f(n)}f(n)} & \mbox{$y(j)$ uniform} &\\
        & \geq \frac{(2^{f(n)}-1)(n-f(n)-1)}{2^{f(n)}f(n)}&\\
        & = \frac{(1-\frac{1}{2^{f(n)}})(n-f(n)-1)}{f(n)}&\\
        & = (\frac{n}{f(n)}-1-\frac{1}{f(n)})(1-\frac{1}{2^{f(n)}}) \in \Omega(\frac{n}{f(n)})&\\
    \end{align*}
\end{proof}

Using this general lower bound on the expected competitiveness we can show different lower bounds. Clearly, $f(n)=1$ yields a high lower bound.

\begin{theorem}
    There is no competitive randomised algorithm that minimises the number of rejected transactions.
\end{theorem}
\begin{proof}
    Follows from Theorem \ref{minRejectedRandom} when setting $f(n)=1$.
\end{proof}


%---------------RESOURCE AUG-------------------------------
\subsection{Resource augmentation}
Since competitive analysis is a worst-case measurement, we consider a different analysis approach called resource augmentation as described in  \cite{Komm:2016:IOC:3036138}. 
%This technique was used for the knapsack problem \cite{IwamaResourceAugmentationKnapsack}, bin-packing \cite{CSIRIK2002308} and machine scheduling \cite{osti_471379}. 
In this approach, an online algorithm may have more resources than the optimal offline algorithm in order to improve the odds of an algorithm against an adversary.
In our setting, we allow the online algorithm to have $h \geq 1$ times more capital on both sides. An online algorithm starts with $\langle hC_l;hC_r \rangle $ if the optimal offline algorithm starts with the initial capital distribution $\langle C_l;C_r \rangle $. In this section, we discuss the existence of deterministic algorithms against different adversary models while considering different values for $h$.

\begin{theorem}
\label{theorem-adaptive-online-resource}
    For $h\leq2$ there is no algorithm that is competitive against any adaptive online adversary.
\end{theorem}
\begin{proof}
    Let the initial capital distribution for the optimal offline algorithm be $\langle C;C \rangle $. Then, an online algorithm starts with $\langle hC;hC \rangle $.
    The first transaction that the adversary presents is $t_1 = (l,r,C)$. If the adversary rejects this transaction, the adversary starts moving $2C$ from right to left back and forth. If the algorithm does not accept these transactions, the adversary keeps giving these transactions such that the algorithm cannot be competitive. If the algorithm decides to move $2C$ first from left to right or first from right to left, then one of the following capital distributions must occur: $\langle (h-2)C;(h+2)C \rangle $ or $\langle (h+2)C;(h-2)C \rangle $. Then, the adversary moves many small transactions from left to right or from right to left accordingly. If $h\leq2$, none of these transactions will be executable. As a result, at most one transaction will be accepted such that rejecting the first transaction is not competitive.
    
    Consequently, an algorithm must accept $t_1$. Then, the new capital distribution is $\langle (h-1)C;(h+1)C \rangle $. Next, the adversary gives the algorithm the transaction $t_2 = (r,l,C)$. If $t_2$ is accepted, the new capital distribution is $\langle hC;hC \rangle $. This scenario is the same as the one described before when rejecting $t_1$. Therefore, the adversary does what we previously described when $t_1$ is rejected which leads here to at most 3 transactions being accepted and the algorithm not being competitive. This implies that an algorithm must reject $t_2$.
    
    If $t_2$ is rejected, the adversary gives the transaction $t_3 = (l,r,C)$. If $t_3$ is accepted the capital distribution is $\langle (h-2)C;(h+2)C \rangle $. Then, the adversary starts moving many small transactions to the right. None of these can then be accepted if $h \leq 2$. In total, three transactions will be accepted. Thus, $t_3$ must be rejected. If $t_3$ is rejected, the adversary shows $t_2$ again. Since it is the same scenario, the adversary shows the transactions as described before. As a result, we conclude that there is no competitive online algorithm for $h\leq2$ that is competitive against any adaptive online adversary.
\end{proof}

\begin{lemma}
    A deterministic online algorithm with $h=2+\epsilon$ and $\epsilon>0$ cannot be better than $\frac{1}{\min(\epsilon,1)}$-competitive against an adaptive online adversary.
\end{lemma}
\begin{proof}
    In the proof of Theorem \ref{theorem-adaptive-online-resource}, we illustrated that an adversary can force that one of the following capital distributions occurs: 
    \begin{enumerate}
        \item $\langle (h-2)C;(h+2)C \rangle$
        \item $\langle (h+2)C;(h-2)C \rangle$
    \end{enumerate}
    Otherwise, an algorithm is not competitive for this setting. When the adversary starts showing small transactions, $\epsilon C$ is left on the side from which the transactions are being sent. Let the capital be $C = n$. Then, $\epsilon n$ capital is left. Let each small transaction move  $1$, then at most $\epsilon n$ transactions are executable. Therefore, the competitive ratio is at least $\frac{1}{\min(1,\epsilon)} = \frac{1}{(\min(1,h-2)}$ (since $c \leq 1$ holds).  
\end{proof}

As shown, there is no competitive online algorithm against an adaptive online adversary for $h\leq2$. Therefore, we focus on algorithms against oblivious adversaries.

\begin{theorem}
    A deterministic algorithm cannot be competitive for $h<2$.
\end{theorem}
\begin{proof}
    Let the initial capital distribution for the online algorithm be $\langle hC;0 \rangle = \langle 2C-\epsilon;0 \rangle$ such that $h = 2 - \frac{\epsilon}{C}$.
    Then, we define the sequences
    \begin{align*}
        &(l,r,C-\frac{\epsilon}{2}), (r,l,1), (r,l,1), \dots, (r,l,1) \\
        &(l,r,C-\frac{\epsilon}{2}), (l,r,C),(r,l,C), \dots, (l,r,C)
    \end{align*}
    Assume there is a competitive algorithm that rejects the first transaction. Then, none of the small movements from right to left can be accepted. This contradicts the assumption and implies that if a competitive deterministic algorithm exists, the first transaction must be accepted.
    Suppose there is a competitive algorithm that accepts the first transaction. Then, the capital distribution after accepting the first transaction is $\langle C-\frac{\epsilon}{2};C-\frac{\epsilon}{2} \rangle$. The movement of $C$ back and forth is not possible anymore and contradicts the assumption that there is a competitive deterministic algorithm that accepts the first transaction. We conclude, that there is no deterministic algorithm for $h = 2 - \frac{\epsilon}{C}$. For $C=n$, $C=2^n$, or even bigger $C$, $h$ goes to $2$ from below. This implies that we can show that there is no competitive deterministic online algorithm for any $h<2.$
\end{proof}
